[Dissertation] Fundamental Limits to Single-Photon Detection

Quantum mechanics cements the intimate relationship between the nature of light and its detection. Historically, quantum theories of photodetection have generally fallen into two categories: the first tries to determine what quantum field observable is measured when photoelectrons are detected, laying the theoretical groundwork for photodetection being possible. The second type are phenomenological theories, which take great care to model the details of specific photodetectors. In this dissertation, we fill in the gap between these two models in the modern literature on photodetection by constructing a fully quantum mechanical and sufficiently realistic model that includes all stages of the photodetection process: transmission, amplification, and a final classical measurement. We accomplish this within the framework of quantum information theory using the language of positive operator valued measures (POVMs). This dissertation contains material previously published in three papers: Propp, Tz. B & van Enk, S. J. (2019). On nonlinear amplification: improved quantum limits for photon counting. Optics Express 27, 16, 23454-23463. Propp, Tz. B & van Enk, S. J. (2019). Quantum networks for single photon detection. Physical Review A, 100, 033836. Propp, Tz. B & van Enk, S. J. (2020). How to project onto an arbitrary single-photon wavepacket. Physical Review A, 102, 053707.

==> union.tex <==
\dedication{This dissertation is the product of unionized labor of the Graduate Teaching
Fellows Federation, AFT Local 3544.}




